On the in vivo recognition of kidney stones using machine learning

Determining the type of kidney stones allows urologists to prescribe a treatment to avoid recurrence of renal lithiasis. An automated in-vivo image-based classification method would be an important step towards an immediate identification of the kidney stone type required as a first phase of the diagnosis. In the literature it was shown on ex-vivo data (i.e., in very controlled scene and image acquisition conditions) that an automated kidney stone classification is indeed feasible. This pilot study compares the kidney stone recognition performances of six shallow machine learning methods and three deep-learning architectures which were tested with in-vivo images of the four most frequent urinary calculi types acquired with an endoscope during standard ureteroscopies. This contribution details the database construction and the design of the tested kidney stones classifiers. Even if the best results were obtained by the Inception v3 architecture (weighted precision, recall and F1-score of 0.97, 0.98 and 0.97, respectively), it is also shown that choosing an appropriate colour space and texture features allows a shallow machine learning method to approach closely the performances of the most promising deep-learning methods (the XGBoost classifier led to weighted precision, recall and F1-score values of 0.96). This paper is the first one that explores the most discriminant features to be extracted from images acquired during ureteroscopies.

==> XAI_Journal_Imgs/Backbones_n_ClassNumber_ProtoPNet.tex <==
\begin{figure*}[] 
    %\begin{center}
    %\centerline{\includesvg[width=\textwidth]{XAI_Journal_Imgs/Backbones_n_ClassNumber_ProtoPNet}}
    \centering
    \includegraphics[width=1.0\linewidth]{XAI_Journal_Imgs/Backbones_n_ClassNumber_ProtoPNet.png}
    \caption{\small{    
    Test Accuracy for different ProtoPNet Backbones and number of classes
    }
    }
    \label{fig:Backbones_n_ClassNumber_ProtoPNet}
    %\end{center}
\end{figure*}
    

==> tables/Backbone_n_ClassNumber_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!h]
\centering
%\resizebox{\linewidth}{!}{%
\scalebox{1.0}{\begin{tabular}{@{}ccccccccccccc@{}}
%\toprule
%\begin{tabular}{cccccccccc}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ProtoPNet   \\      with backbone:\end{tabular}} &
  \multicolumn{3}{c}{Accuracy 4 classes} &
  \multicolumn{3}{c}{Accuracy 5 classes} &
  \multicolumn{3}{c}{Accuracy 6 classes} \\
 &
  Surface &
  Section &
  Mixed &
  Surface &
  Section &
  Mixed &
  Surface &
  Section &
  Mixed \\ \hline
Resnet18 &
  87.37\% &
  79.62\% &
  83.13\% &
  \textbf{89.00\%} &
  79.70\% &
  84.95\% &
  \textbf{81.17\%} &
  70.50\% &
  76.12\% \\
Resnet50 &
  89.75\% &
  74.88\% &
  84.94\% &
  85.20\% &
  \textbf{81.40\%} &
  84.10\% &
  80.08\% &
  \textbf{72.17\%} &
  76.46\% \\
Resnet152 &
  87.00\% &
  \textbf{80.50\%} &
  \textbf{85.25\%} &
  81.20\% &
  81.30\% &
  \textbf{85.60\%} &
  77.17\% &
  \textbf{72.17\%} &
  77.29\% \\
VGG16 &
  89.75\% &
  73.62\% &
  84.94\% &
  87.60\% &
  75.80\% &
  84.05\% &
  75.50\% &
  70.58\% &
  75.08\% \\
VGG19 &
  \textbf{92.00\%} &
  75.25\% &
  83.87\% &
  82.40\% &
  74.80\% &
  82.95\% &
  78.08\% &
  69.33\% &
  74.58\% \\
DenseNet201 &
  89.75\% &
  80.00\% &
  81.69\% &
  86.90\% &
  79.00\% &
  85.35\% &
  79.42\% &
  70.50\% &
  \textbf{77.88\%}
\end{tabular}
}
\caption{Test Accuracy for different ProtoPNet Backbones and number of classes}
\label{table:Backbones_varingClassw}
\end{table*}

